Enhancing the Security & Privacy of Wearable Brain-Computer Interfaces

Brain computing interfaces (BCI) are used in a plethora of safety/privacy-critical applications, ranging from healthcare to smart communication and control. Wearable BCI setups typically involve a head-mounted sensor connected to a mobile device, combined with ML-based data processing. Consequently, they are susceptible to a multiplicity of attacks across the hardware, software, and networking stacks used that can leak users' brainwave data or at worst relinquish control of BCI-assisted devices to remote attackers. In this paper, we: (i) analyse the whole-system security and privacy threats to existing wearable BCI products from an operating system and adversarial machine learning perspective; and (ii) introduce Argus, the first information flow control system for wearable BCI applications that mitigates these attacks. Argus' domain-specific design leads to a lightweight implementation on Linux ARM platforms suitable for existing BCI use-cases. Our proof of concept attacks on real-world BCI devices (Muse, NeuroSky, and OpenBCI) led us to discover more than 300 vulnerabilities across the stacks of six major attack vectors. Our evaluation shows Argus is highly effective in tracking sensitive dataflows and restricting these attacks with an acceptable memory and performance overhead (<15%).

==> 7-discussion.tex <==
\section{Discussion}

\textbf{improving the framework}

\textbf{Other adversarial attacks.}
Our adversarial attack PoCs are a subset of bigger categories representing white- and black-box attacks. Therefore, attack vectors can be extended to other state-of-the-art approaches such as DeepFool or Carlini-Wagner, other poisoning or extraction attacks as well as attacks specific to the platform or application in consideration. Moreover, while current deep learning approaches on resource-constrained devices focus mainly on inference, recent works are exploiting few-shot learning and personalization methods to perform training on-device. These new paradigms introduce new attack vectors to consider for training time auditing. In addition, there are new attacks introduced at a high speed, therefore only an extensible approach can handle such expansion.  With the right considerations, \tool can be extended to investigate these new sources of vulnerability.

Finally, the majority of adversarial attacks that are now considered in literature come from the computer vision community. The signals received from the BCI devices are different and, consequently, need special attention and investigation. As we saw in \S~\ref{fig:clean_adv}, an adversarial perturbation than can be considered as a high strength perturbation in an image input (i.e. visible to the naked eye) might not be so for the EEG signal. Moreover, further studies are needed to include the plethora of attacks stemming from time series signal (such as EEG) manipulation in the time and frequency domain.



==> application.tex <==
\subsection{3D Block Stacking Application}
\label{sec:app}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 80 CHAR %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\raj{merge this into the evaluation section for the user study}

To evaluate the usability of {\myit} on a real application at the user level,
we designed an AR application for implicitly measuring the stereoscopsis level 
of children with strabismus using AR HMDs, and performed an Institutional Review
Board (IRB)-approved pilot study with strabismus (i.e., crossed eye) patients in
the ophthalmology department at a university hospital.
%
The purpose of our pilot study was to validate changes in user-perceived
object rendering quality when applying {\myit} with different configurations.


Traditionally, devices such as keratometers are used to measure the 
stereoscopsis level. However, these devices are bulky and cannot effectively 
gain the attention of children to focus during the measurements.
%
For this reason, the clinical staff asked for a more interactive and engaging 
game to measure children's stereoscopsis levels, and we designed an AR-based 
game where the children were asked to stack 3D blocks using Microsoft HoloLens%
\footnote{We used DirectX as the underlying native graphics library}
(c.f., \fig\ref{fig:hololens}).


The block stacking game operates as follows.
%
When the application starts, a white cube palette is displayed.
Once the user visually focuses on the cube, the user is asked to press a clicker
device and move the object in the 3D space.
%
Using such movements, the user is asked to stack all cube blocks on the display.
The performance of moving the objects becomes an indirect measure of the 
stereoscopsis level. 
%
We designed this game and user study to confirm if {\myit} makes proper 
transitions in frame rate or changes in object quality, while minimally 
affecting the user perceived quality.
%
Furthermore, we also gathered statistics on the amount of energy 
that can be saved by applying {\myit} to real-world applications%
\footnote{A sample video of the application and its interaction with {\myit} is
available, and we will provide the URL after the anonymous review process.
%at \todo{http://}
}.

%\jk{Let's make a recording of the task and share on Youtube.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% 이러한 실제 stereoscopsis의 측정에 앞서, 우리는 AR HMD의 사용성에 대해서 면밀히 검토할 필요가 있었다. 특히 우리의 실험 대상은 어린이 환자들이었고, 이러한 환자들이 새로운 환경인 HMD 환경을 쉽게 이용할 수 있는지는 큰 챌린지 중 하나였다. 구체적으로 살펴보면 첫번째로 조작의 편의성을 확인해야 했다. Microsoft HoloLens로 조작할 수 있는 주요 방법은 손가락을 통한 gesture 인식과 external 장비인 clicker 가 있다. gesture 인식의 경우 HoloLens에 부착되어 있는 depth sensor에 손이 보여야 하는 문제가 있고 클릭의 정밀도가 낮다는 단점이 있는 반면, clicker를 이용하면 click 이라는 액션이 명확하다는 장점이 있기 때문에 우리는 clicker를 사용하기로 했다. 두번째로 HMD라는 경험이 환자들에게 어떻게 느껴지는지 인 지점이 있었다. 알려져 있기로 HMD 경험이 눈의 고통을 주기도 하고, 어지러움을 야기할 수도 있고, 불편함을 주기도 했는데 실제로 어린이 환자에게 AR 응용을 적용됐을 때 어떤 경험을 주는지 확인해 보는 것은 추후 AR 응용을 개발하는데에 좋은 information이 될 수 있다.  마지막으로 어린이 환자를 위한 측정 방법과 설문의 난이도를 고려하는 것이 중요했다. block stacking이라는 간단한 동작이지만 이러한 동작이 어린이들, 특히 환아들에게 어려울 수 있고 이러한 과정에 대한 설문을 하는 과정도 쉬운 언어를 통해서 진행이 되어야 했다.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 80 CHAR %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Application-level View Frustum Culling}

% 이번 섹션에서는 draw call을 줄이기 위한 방법인 user level view frustum culling의 방법에 대해 구체적으로 설명한다. 이전 섹션에 말했 듯, culling은 visibility를 판단하는 작업이다. 그래픽스 파이프라인에서는 view frustum culling이라고 불리는 작업을 수행하는데, 이는 카메라 정보, 그 중에서도 종횡비 시야각, 그리고 최소 가시거리, 최대 가시거리 정보를 통해 frustum을 만들고, 렌더링하는 물체들이 frustum의 바깥으로 나가는지 그렇지 않은지를 판단하는 방법들이다. 이러한 방법을 통해 화면에 보이지 않는 triangles를 판단하고, 이후 pipeline 작업에서는 해당 triangles를 배제해서 성능 향상을 이룬다.

% 하지만 그럼에도 불구하고 system level이 아닌 application level에서의 view frustum culling은 필요하다. 그 이유는 렌더링 되지 않는 draw call도 에너지 소모에 영향을 주기 때문이다. 그 이유는 view frustum culling이 일어나는 시점의 문제에 있다. draw call이 불리면 graphics pipeline은 모든 그려야 하는 vertices를 vertex shader를 통해서 병렬적으로 transformation한다. 이 이후 시점에서 view frustum culling이 일어난다. 즉, 실제로 그려지게 될지 모르는 상태에서 연산을 해야 한다는 것이다. 이로 인해 높은 the number of triangles를 가진 모델의 경우 자원을 크게 낭비하게 된다.

% 우리는 다음과 같은 방법을 통해 user level에서 light-weight view frustum culling을 진행한다. gpu에서의 view frustum culling은 mesh의 모든 triangles에 대해서 진행되기 때문에 비용이 비싸다. 하지만 우리는 우리는 mesh의 triangles가 아닌 initialization 시에 만든 mesh의 bounding box를 이용한다. 이러한 bounding box는 모델의 전체를 bound하고 있기 때문에 만약 camera가 바라보고 있는 방향기준으로 시야각 바깥에 bounding box가 있다면 이 모델이 보일 가능성이 없다고 생각할 수 있다. 이러한 케이스에 대해서는 해당 모델에 대한 draw call을 호출하지 않음으로 인해서 에너지 소모를 줄일 수 있다.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 80 CHAR %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

To explain the implementation details of the bounding box projection process, we take as example, once again, the Stanford Bunny. Say that there is a Stanford Bunny and we want to compute the three metrics (i.e., XXX, XXX, and XXX) discussed above. Given the vertices and topology information for the bunny rendering, we receive the transformation matrix from the application to apply the target transformation (e.g., scaling, rotation, translation) to the vertices. On the application's perspective, as a result of the transformation process, a vertex $V$ will be located at $(x,y,z)$ from the origin point $(0,0,0)$. Here we say that $V$ is transformed in to world-space. \jk{huh???}

% 간단한 예로 화면에 stanford bunny가 그려져 있고, 우리가 위에서 정의한 세가지 방법들을 계산하기 위해 유저 입장에서 이 bunny가 어떻게 보이는지를 계산하고 싶다. 렌더링을 하기 위한 vertices와 topology information이 있을 때, 이에 원하는 transformation (e.g. scaling, rotation, translation)을 적용하기 위해 transformation matrix를 application 단으로부터 받아서 vertices에 곱해준다. 이렇게 transform된 vertices는 중 하나의 vertices v 는 application 입장에서 origin, 즉 (0, 0, 0)을 기준으로 (x, y, z)에 위치하게 된다. 이때의 v를 v is transformed into world space. 라고 표현한다. 이 상태에서는 user 의 

\end{comment}




==> attackvectors.tex <==
\begin{table*}[htb]
  \centering
  \footnotesize
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{|c|l|l|c|}
      \hline

    & \bf Attack Vector       & \bf Impact  & \bf \tool \\
    \hline
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\bf Systems and userspace}}}
    
    &  &  &\chk \\
    &  &      & \chk \\
    &  &       & \chk \\
    &  &     &  \chk\\
    &  &     & \chk \\
    
    &  &  unsafe native bindings     & \chk \\

    &  &  Heartbleed bug     & \chk \\ 
  
    \hline
    
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\bf Adverserial ML}}}

                &  && \\


     &  &   &   \\
      &  &  & \\

    \hline
    

  \end{tabular}}
  \caption{.}
  \label{cvetab}
\end{table*}


==> avs-evals.tex <==
\begin{table}
    \begin{tabular}{|l|l||l|l|}
    \hline
    Attack vectors & NuroSky & Muse & OpenBCI \\ \hline
    AV1            & ~       & ~    & ~       \\
    AV2            & ~       & ~    & ~       \\
    AV3           & ~       & ~    & ~       \\ \hline
    \end{tabular}
    \caption{The number of attack PoCs from/to the host that we implemented in different BCI frameworks.}
\end{table}

==> domains.tex <==




\begin{table*}[htb]
  \centering
  \footnotesize
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{|l|l|l|}
    \hline
    Feature                   & ARM Memory Domains                             & Intel MPK                                                            \\ \hline
    Per process domains       & 16                                             & 16                                                                   \\ \hline
    Access control register   & DACR  (2 bits per domain, privileged register) & PKRU (2 bits per domain, userspace register)                         \\ \hline
    Access rights             & No-access, Full access, MMU default            & No-access, write-disable, MMU default                                \\ \hline
    Paging modes              & 2-level paging (bits 8:5, level 1 entries)     &  4-level paging (bits 62:59 of PDPTE)                                \\ \hline
    Address space privilege   &  Privileged \& usersapce                       &  Userspace only                                                      \\ \hline
    Specific page fault       & Domain fault                                   & PK fault                                                             \\ \hline
    Kernel virtual memory API & No support                                     & Limited support (\texttt{pkey\_mprotect}, \texttt{pkey\_alloc}, \texttt{pkey\_free}, and \texttt{mmap}) \\ \hline
    \end{tabular}}

    \caption{ARM memory domains vs Intel MPK: Despite being efficient building blocks of isolation, such features have various limitations that \textmu Tiles abstraction resolves to provide effective intra-process privilege separation.}
    \label{mpk}
\end{table*}

\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%

    \begin{tabular}{|l|l|l|}
    
    \hline
    Mode & Bits & Description                                                                     \\ \hline
    No Access   & 00 &  Any access causes a domain fault.                          \\\hline
    Manager     & 11 & Full accesses with no permissions check.\\\hline
    Client      & 01 &  Accesses are checked against the page tables   \\\hline
    Reserved    & 10 &   Unknown behaviour. \\ \hline
    \end{tabular}}
    \caption{ARM memory domains access permissions }
    \label{domains}
\end{table}







==> figures/FGSMMedianFilter.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]
\begin{adjustbox}{width=1.2\textwidth,center=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & FSGM \%Acc NO Squeezing & FSGM \%Acc WITH Squeezing & \%change post Squeeze \\ \hline
3  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}6.20\%  & +1.1\%  \\ \hline
5  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}8.40\%  & +3.3\%  \\ \hline
7  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}11.10\% & +6\%    \\ \hline
9  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}15.10\% & +10\%   \\ \hline
11 & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}18.60\% & +13.5\% \\ \hline
13 & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}21.90\% & +16.8\% \\ \hline
15 & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}25.10\% & +20\%   \\ \hline
17 & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}27.70\% & +22.6\% \\ \hline
19 & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}32.20\% & +27.1\% \\ \hline
\end{tabular}
\end{adjustbox}
\caption{FSGM Squeezing Results using a Median Filter}
\end{table}

==> figures/FGSMMovingAverage.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]
\begin{adjustbox}{width=1.2\textwidth,center=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & Acc NO Squeezing & Acc WITH Squeezing & \%change post Squeeze \\ \hline
2  & 5.10\%                         & \cellcolor[HTML]{FFFFFF}6.70\%  & +1.6\%  \\ \hline
3  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}7.60\%  & +2.5\%  \\ \hline
4  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}10.40\% & +5.3\%  \\ \hline
5  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}11.20\% & +6.1\%  \\ \hline
6  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}12.90\% & +7.8\%  \\ \hline
7  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}14.60\% & +9.5\%  \\ \hline
8  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}16.30\% & +11.2\% \\ \hline
9  & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}18.80\% & +13.7\% \\ \hline
10 & \cellcolor[HTML]{FFFFFF}5.10\% & \cellcolor[HTML]{FFFFFF}21.10\% & +16\%   \\ \hline
\end{tabular}
\end{adjustbox}
\caption{FSGM Squeezing Results using Moving Average}
\end{table}

==> figures/FGSMSavgolFilter.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]
\begin{adjustbox}{width=1.2\textwidth,center=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & Acc NO Squeezing & FSGM Acc WITH Squeezing & change post Squeeze \\ \hline
(7, 5)  & 5.10\% & 5.30\%  & +0.2\% \\ \hline
(11, 5) & 5.10\% & 6.20\%  & +1.1\% \\ \hline
(15, 5) & 5.10\% & 7.90\%  & +2.8\% \\ \hline
(19, 5) & 5.10\% & 10.30\% & +5.2\% \\ \hline
(23, 5) & 5.10\% & 12.60\% & +7.5\% \\ \hline
(11, 9) & 5.10\% & 5.20\%  & +0.1\% \\ \hline
(15, 9) & 5.10\% & 5.40\%  & +0.3\% \\ \hline
(19, 9) & 5.10\% & 6.10\%  & +1\%   \\ \hline
(23, 9) & 5.10\% & 6.80\%  & +1.7\% \\ \hline
(27, 9) & 5.10\% & 8.50\%  & +3.4\% \\ \hline
\end{tabular}
\end{adjustbox}
\caption{FSGM Squeezing Results using Savgol Filtering}
\end{table}

==> figures/FGSM_Table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]
\begin{adjustbox}{width=1.2\textwidth,center=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{6}{c}{FGSM Epsilon} \\ \cline{1-1}
STD & 0 & 0.01 & 0.02 & 0.03 & 0.04 & 0.05 \\
0 & \cellcolor[HTML]{FFFFFF}59.9\% & \cellcolor[HTML]{FFFFFF}18.7\% & \cellcolor[HTML]{FFFFFF}2.0\% & \cellcolor[HTML]{FFFFFF}0.0\% & \cellcolor[HTML]{FFFFFF}0.0\% & \cellcolor[HTML]{FFFFFF}0.0\% \\
0.1 & \cellcolor[HTML]{FFFFFF}60.1\% & \cellcolor[HTML]{FFFFFF}19.8\% & \cellcolor[HTML]{FFFFFF}2.2\% & \cellcolor[HTML]{FFFFFF}0.2\% & \cellcolor[HTML]{FFFFFF}0.0\% & \cellcolor[HTML]{FFFFFF}0.0\% \\
0.3 & \cellcolor[HTML]{FFFFFF}51.7\% & \cellcolor[HTML]{FFFFFF}22.9\% & \cellcolor[HTML]{FFFFFF}5.0\% & \cellcolor[HTML]{FFFFFF}0.6\% & \cellcolor[HTML]{FFFFFF}0.0\% & \cellcolor[HTML]{FFFFFF}0.0\% \\
0.5 & \cellcolor[HTML]{FFFFFF}52.3\% & \cellcolor[HTML]{FFFFFF}26.7\% & \cellcolor[HTML]{FFFFFF}7.9\% & \cellcolor[HTML]{FFFFFF}1.6\% & \cellcolor[HTML]{FFFFFF}0.0\% & \cellcolor[HTML]{FFFFFF}0.0\% \\
1 & \cellcolor[HTML]{FFFFFF}50.8\% & \cellcolor[HTML]{FFFFFF}25.1\% & \cellcolor[HTML]{FFFFFF}10.5\% & \cellcolor[HTML]{FFFFFF}2.4\% & \cellcolor[HTML]{FFFFFF}1.0\% & \cellcolor[HTML]{FFFFFF}0.1\%
\end{tabular}
\end{adjustbox}
\caption{FSGM Squeezing Results using a Median Filter}
\end{table}

==> figures/PGD_Table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]
\begin{adjustbox}{width=1.2\textwidth,center=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{6}{c}{PGD Iterations} \\ \cline{1-1}
STD & 0 & 1 & 2 & 3 & 4 & 5 \\
0 & \cellcolor[HTML]{FFFFFF}59.9\% & \cellcolor[HTML]{FFFFFF}12.0\% & \cellcolor[HTML]{FFFFFF}1.3\% & \cellcolor[HTML]{FFFFFF}0.2\% & \cellcolor[HTML]{FFFFFF}0.0\% & \cellcolor[HTML]{FFFFFF}0.0\% \\
0.1 & \cellcolor[HTML]{FFFFFF}65.9\% & \cellcolor[HTML]{FFFFFF}13.3\% & \cellcolor[HTML]{FFFFFF}1.7\% & \cellcolor[HTML]{FFFFFF}0.3\% & \cellcolor[HTML]{FFFFFF}0.0\% & \cellcolor[HTML]{FFFFFF}0.0\% \\
0.3 & \cellcolor[HTML]{FFFFFF}58.8\% & \cellcolor[HTML]{FFFFFF}18.0\% & \cellcolor[HTML]{FFFFFF}2.3\% & \cellcolor[HTML]{FFFFFF}0.0\% & \cellcolor[HTML]{FFFFFF}0.0\% & \cellcolor[HTML]{FFFFFF}0.0\% \\
0.5 & \cellcolor[HTML]{FFFFFF}62.1\% & \cellcolor[HTML]{FFFFFF}22.2\% & \cellcolor[HTML]{FFFFFF}5.2\% & \cellcolor[HTML]{FFFFFF}0.6\% & \cellcolor[HTML]{FFFFFF}0.1\% & \cellcolor[HTML]{FFFFFF}0.0\% \\
1 & \cellcolor[HTML]{FFFFFF}51.0\% & \cellcolor[HTML]{FFFFFF}26.7\% & \cellcolor[HTML]{FFFFFF}8.1\% & \cellcolor[HTML]{FFFFFF}3.4\% & \cellcolor[HTML]{FFFFFF}0.8\% & \cellcolor[HTML]{FFFFFF}0.3\%
\end{tabular}
\end{adjustbox}
\caption{FSGM Squeezing Results using a Median Filter}
\end{table}

==> imp-temp.tex <==

\subsection{Background: ARM memory managment}\label{tzencs}



\input{domains.tex}
\subsection{HW-enforced VMA Tagging}\label{memdomain}

Modern CPUs have supported memory protection mechanisms that are more efficient than traditional paging. For example, VMA tagging features such as Intel Memory Protection Keys~\cite{mpk} and ARMv7 Memory Domains (MDs)~\cite{arm2012architecture} provide fast isolation by reducing page table walks and TLB flushes. Though the implementations across Intel and ARM vary considerably (see Table~\ref{mpk}), \textmu Tiles high-level VM abstraction can securely utilize these efficient building blocks while hiding their limitations.  In this paper, we primarily describe the design of \textmu Tiles for ARMv7-A that is a widely used CPU in IoT and mobile devices. Also, ARM-MD is a less flexible and more challenging interface to support (\S\ref{challenges}) that covers most MPK limitations as well.

As a summary of ARMv7-A memory management, page table entries consist of a virtual base address, a physical base address, Address Space Identifier (ASID) tags, domain IDs, and a set of flags for access control and other page attributes. It supports a two-level hierarchical page table when using a short-descriptor translation table format, and supports variable page sizes (1GB, 1MB, 64KB, and 4KB).
ARM supports two page tables simultaneously, using the hardware registers TTBR0 and TTBR1. A virtual address is mapped to a physical address by the CPU, depending on settings in TTBRC. This control register has a field that sets a split point in the address space. Addresses below the cutoff value are mapped through the page tables pointed to by TTBR0 (used per process), and addresses above the cutoff value are mapped through TTBR1 (used by the kernel). \\
The translation tables hold a four-bits \textbf{domain ID} ranging from $D0$ to $D15$. Access control for each domain is handled by setting a domain access control register (DACR) in $CP15$, which is a 32-bit register only accessible in the privileged processor modes. Each domain is assigned two bits in DACR, which defines its access rights. \\
The four possible access rights for a domain are No Access, Manager, Client, and Reserved (see Table~\ref{domains}). Those fields let the processor ~\rom{1} prohibit access to the domain mapped memory--No Access;~\rom{2} allow unlimited access to the memory despite permission bits in the page table-- Manager; or~\rom{3} let the access right be the same as the page table permissions--Client. Any access violation causes a domain fault. Changes to the DACR are low cost and activated without affecting the TLB. Hence changing domain permissions does not require TLB flushes. 


\subsection{Challenges of Utilizing ARM-MD}\label{challenges}
Though ARM memory domains are a promising primitive in concept, the current hardware implementation and OS support suffer from significant problems that have prevented their broader adoption:\\
\noindent\textbf{Scalability:} ARM relies on a 32-bit DACR register and so supports only up to 16 domains. Allocating a larger register (e.g., 512 bits) would mean larger page table entries or additional storage for domain IDs.\\
\textbf{Flexibility:}
Unlike Intel MPK, ARM-MDs only apply to first-level entries; the second-level entries inherit the same permissions. This prevents arbitrary granularity of memory protections to small page boundaries and reduces the performance of some applications~\cite{cox2017efficient}.
Also, the DACR access control options do not directly mark a domain as read-only, write-only, or exec-only. So the higher-level VM abstraction should resolve these issues.\\
\textbf{Performance:} Changing the DACR is a fast but privileged operation, so any change of domain access permissions from userspace require a system call. This is unlike Intel MPK that makes its Protection Key Rights Register (PKRU) accessible directly from userspace.\\
\textbf{Userspace:} There is no Linux userspace interface for using ARM-MD; it is only used within the kernel to map the kernel and userspace into separate domains. In contrast, Linux already provides some basic support for utilizing Intel MPK from userspace.\\
\textbf{Security:} Though the DACR is only accessible in privileged mode, any syscall that changes this register is a potential breach that could cause the attacker to gain full control\footnote{An occasion that has happened once already through the misuse of the put\_user/get\_user kernel API (CVE-2013-6282)}. Also, since only 16 domains are supported, it is trivial to guess other domains' identifiers, making it essential to not expose these directly to application code.



\subsection{Enforcing Isolation}\label{sec:isolation}


\paragraph{Local monitors: dataflow checks.}
% 
\tool partitions both the Linux kernel and TEE runtime to dynamically redirect every call on a tagged object to a separated path toward its associated monitors.
%Note that in-enclave runtime usually manages fewer objects than the kernel, such as enclave's memory, threads, and IPC/RPC. 
% 
Since the in-enclave runtime is trusted, the \ssm doesn't need to monitor the runtime and protect \sem.
% 
%On the other hand, the \skm enforces safe dataflows for the host objects.
% 
However, the kernel is not trusted. Thus, the \skm only handles the dataflow \textit{checking} operations. 
% 
When the \skm wants to \textit{change} dataflows by creating or updating labels and capability lists, it has to request \ssm. 
% 
Each monitor implements a single set of DIFC rules that checks secrecy and integrity dataflows of given objects including threads. For each compartment, \tool's proxy in the syscall exception handler traps and redirects the calls to \skm (L3, code~\ref{code3}). 
Within each monitor, \tool performs a lookup over the object (L6). Depending on the object and thread's labels and capability lists, its associated monitor checks DIFC rules (L8-13). 
% 
For each kernel object, we extend its main data structure with a pointer to a metadata which holds the object's label (e.g., \texttt{inode->s\_obj\_label}). For in-enclave compartmentalization we trust \sem to hold this metadata, but for kernel objects each metadata is mapped \texttt{read-only} to protected memory by the \ssm (via a shadow address space~\cite{song2016enforcing}) so the kernel cannot manipulate it. %When creating a labeled object, \skm assigns a metadata and forward the call to the kernel (or in-enclave runtime) for creating the object.




\paragraph{Local monitors: virtual address partitioning.}

%\todo{
%virt mem is used for a lot stuff, kernel manages it as it wants. how we are introducing a second layer. 
%- how is it safe?
%- why doesnt it break the kernel?
%- two competing managers who dont trust each other 
%what about copy on write, shared memory for forking, memory mapped io, }
% 
To enforce intra-address space isolation of objects, \tool extends the existing VM (virtual memory) layers (for both the kernel and TEE runtime) with a new VM abstraction. It provides a lightweight slab allocator, memory management (e.g., \texttt{s\_mmap,s\_mprotect}, etc.), and a fault handler dedicated to \tool contiguous memory objects. This layer uses kernel functionalities for initializing its heap with a dedicated region. This avoids breaking the kernel memory management for regular applications; however, the monitor's functionality is independent of kernel memory management. \tool limits accessing or changing its memory objects by~\rom{1} tracking and mapping them to dedicated virtual page tables;~\rom{2} tracking tagged threads and~\rom{3} adding security hooks within the kernel/runtime VM and VFS layers to redirect any calls from a tagged thread or within the protected memory regions to its associated monitor for dataflow checking. 

Each monitor has to track its local tagged threads. For each thread, \tool maintains the metadata for labels, capability lists, and memory objects. 
For easy tracking, \tool extends the main task data structure (e.g., \texttt{task\_struct} in Linux) with a pointer to the metadata. \codename assigns labels to every block of VA objects and not every page to avoid a large overhead (similar to segmentation). Note that both the host application and enclave can create VA objects for compartmentalizing their private data.
% 
The \tool VA abstraction layer maintains its own virtual page tables (similar to \texttt{pgd\_t} structure) per thread.
% 
When a thread needs to operate on the memory object, \tool performs a lightweight context switch to lazy-map the thread's virtual page table to the \texttt{TTBR/CR3} register.
% 
\tool uses ACID/PCID tags to ensure that the page tables are not mapped to overlapping memory and do not incur expensive TLB flushes. 
% 
%Further, similar to other objects, for each VA object \tool maintains metadata information about address space range, label, and permissions which is read-only for the kernel (\texttt{s\_mem\_obj} in Appendix A:\cref{imcstruct}). 
% 
%\todo{add an example to the above for memory mapped file? or just a buffer on the heap, schematic figure with data structs and pointers
%- why cant the kernel change the pointer to the metadata struct and point it to its own struct
%}

\input{listings/code3}

\paragraph{Sharing while preserving ownership.}
In general, sharing resources between an enclave and its host application is not safe and not supported by several TEEs, including SGX enclaves. However, the mutually distrustful nature of \tool enables sharing resources per-\td or per-thread while each enclave or application thread can preserve its control over shared objects. 
% 
For example (Figure~\ref{fig:shm}), an enclave thread $e$ creates a memory object $M_{1}$ as read-only and grants the access capability ($t^+$) to the application thread $p$. Hence, only $p$ can read from $M_{1}$, but it cannot change $M_{1}$ layout or permissions since $m1 \notin D_{p}$. Other threads in the same process or enclave cannot access $M_{1}$ (e.g., threads $d$ or $c$ in Figure~\ref{fig:shm}). 
% 

\begin{figure*}[t]
\centering
\includegraphics[scale=.5]{bvisor/figures/higharch3.pdf}
\caption{Shared memory between an enclave and app}
\label{fig:shm}
\squeezeup

\end{figure*}


\paragraph{Secure delegation \& monitoring with \ssm.}
% 
\tool restricts the kernel to either refuse to perform redirecting calls to \skm for dataflow checking or abuse them to evade detection. 
% why such small amount of checking is sufficient
First, \tool partitions critical paths of tagged and non-tagged objects to limit an unauthorized kernel thread from accessing, modifying, or transferring the labeled objects directly. Second, 
 the \ssm ensures that the kernel performs the expected checks through several steps. \nom{1} in the secure boot process, \ssm only loads a verified kernel and monitors. \nom{2} for runtime protection, \ssm page tables dual-map parts of the physical address spaces with the kernel to create shadow address space regions such that the kernel has read-only access to them.
 %~\footnote{Side channel attacks over page tables are out of scope.}
 Thus, any call or event that change the labels/capabilities are trapped immediately to the \ssm for updating the isolated metadata that holds the label or capability list within the shadow region. Further, the \ssm checks associated kernel threads' label and capability lists to detect API misuses. 
\nom{3} \ssm uses the shadow regions to map critical parts of the kernel (e.g., the .text, read-only data sections, page-table base addresses) as read-only. The \ssm is thus notified if an attacker tries to disable or jump over \tool security hooks by tampering with the kernel code or injecting an unauthorized kernel module. \nom{4} \ssm monitors events that lead to violating shadow regions like changing page tables or disabling the MMU by its instruction emulator that traps sensitive instructions within the regions (e.g., MCR, LDC, STP). It also uses event-driven monitoring of the kernel's static invariants (e.g., syscall tables, exception vectors). 
The \ssm guarantees that the vulnerabilities in the kernel cannot cause data-only attacks to bypass the security hooks by ensuring the data pointers are located within the shadow regions.
These measures and techniques are partly inspired by state-of-the-art kernel monitoring schemes (e.g., Samsung KNOX~\cite{azab2014hypervision}, KENALI~\cite{song2016enforcing}). But, these are only practical since \tool has well-defined verifiers (one set of simple rules for all objects), and a small \ssm and \skm with few verifiable security hooks.
% 
We refer to the exact security arguments for this claim to Section~\ref{sec:security}.


% \paragraph{SSM.}
% the enclave rt and the untrusted kernel together are expected to manage these labels and enforce the expected isolation. 
% % why do we still want the kernel to do it?
% the enclave rt and the host kernel are the right place to do this because they are the right abstraction, have direct access to the objects, reduces the size, etc. 
% 
% this is a lot of sw logic (e.g., flume is 30k
% 
% rt is trusted and is expected to do its part of checks, its small, and is part of the tcb anyway. 
% 



% 
% Such decoupling of label management is ?
% % 
% What remains is to actually enforce the isolation as per the labels.
% 

% \paragraph{\tool Kernel Module.}
% since \tool maps all its objects as \imc at the virtual address level, it can easily leverage underlying hardware isolation mechanisms to enforce the expected isolation. 
% % 
% to do this, the ssm converts the labels into rules and configures the hardware accordingly. 
% % 
% this way \sirius does not have to rely on the kernel to do the  isolation, instead the hardware enforces the labels at runtime. 
% % 
% \codename isolates different types of \imc 
% via combination of intra-address space memory protection and per-object dataflow controlling.
% % 
% Specifically, \codename adds an abstraction over contiguous regions of virtual memory (VM) and utilizes existing hardware features (e.g., MMU, TZ, memory domains) to isolate each region.  
% % 
% The type of isolation is configurable when creating a region (via \texttt{vao\_create} flags). 
% More importantly, \codename manages capabilities mappings and checks dataflow rules for each object. 
% 

% \paragraph{\tool components.}
% introduce/remind about the in-enclave kernel, in-enclave checker, driver, host kernel, host checker, smm parts that are added/modified by \tool
% % 
% what is trusted and untrusted by whom (maybe already covered somewhere? remind here)



% 
% in this sense, the checking is distributed.
% 
% without the inenclave checker, it is impossible to do checks within the enclave.

%\paragraph{Explicit Labels.}
% Mapping labels \& capabilities to \imc.}
% 
%\codename internally maintains a label and capability list per object and locates security hooks in essential places at their associated abstractions (e.g., VFS, network layer, thread management) to ensure isolation via safe dataflow. \codename ensures its APIs and all necessary sycalls routed through these checks. Its virtual memory abstraction added on top of the existing VM layer and enforces correct access and changes to each \vao.
%\codename checks the dataflows before any potential access control mechanism (e.g., DAC, MAC) that may already be enabled so attackers can not bypass the checks through those. Note that the kernel is untrusted as we explain here later on how our \ssm protects label and capability changes and monitors the kernel.




%\paragraph{Implicit Labels.}
% ing virtual memory objects }
% 
%\codename assigns labels to every block of \vao and not every page to avoid a large overhead. Note that both the host application and enclave can create \vao{s} for compartmentalizing their private data.When a thread has the $\theta^{+}$ capability for \vao $\theta$, it gains the privilege to access the \vao with the default permission set by the owner in creation time. For instance, in code sample~\ref{code}, \texttt{mem\_obj[2]} default permission is \texttt{readonly}. Without having $\theta^{-}$, declassification capability, a thread is not allowed to change a \vao permission (\texttt{imc\_mprotect}), modify its memory layout by adding/removing pages (via \texttt{imc\_mmap/munmap}), or transfer the content to untrusted sources (e.g., memcpy, copy to a file, or share with other thread). 


%song2016enforcing,liljestrand2019pac





==> listings/code.tex <==
\begin{lstlisting}
static int fn(void* arg) {
  s_execv(mem_obj[1],zlib,deflateInit,Z_DEFAULT_COMPRESSION);
}
void threading_test (void) {
  int cid= s_create(SLABEL);
  int fd= open(tmpname,O_CREAT);
  s_add (cid,persistent_file,fd);
  mem_obj[1] = s_vao_create(DEFAULT, MEMDOM_READ|MEMDOM_WRITE);
  mem_obj[2] = s_vao_create(HW_MD,MEMDOM_READ);
  s_add(cid,vao,memory_obj[1],memory_obj[2])
  // map VA objects to threads
  tid1 = s_clone(cid, mem_obj[1],&fn ,...);
  tid2 = s_clone(cid, mem_obj[2],...);
  s_wait(&status);
  s_cleanup(cid );
}
  
\end{lstlisting}











==> listings/code2.tex <==
\begin{lstlisting}%[caption={Pseudocode of MCA API: example of IMC memory operations.},captionpos=b,label={code2}]

void imc_threading_test (void) {
//initialization ....
    td_id= td_create(SLABEL);//create a TD
    imc_id = imc_create(DEFAULT);// create an IMC
    s_grant(self, imc_id,
              MEMDOM_READ | MEMDOM_WRITE);
    td_map(imc,imc_id); //map imc to a TD    
    /* allocate memory from imc */
    private_blk = (char*) imc_malloc(imc_id, len);
    /* make imc inaccessible */
    s_access_disable(imc,imc_id);
    //... untrusted computations ....//
    /* make imc accessible */
    s_access_enable(imc,imc_id);
    //... trusted computations ....//
    /* cleanup imc */
    imc_free(private_blk);
    td_kill(td_id);
//the rest....}  
\end{lstlisting}



==> listings/code3.tex <==



\begin{lstlisting}[caption={Pseudocode of dataflow checking by KM},captionpos=b,label={code3}]
/// syscall handler ///
SYSCALL_DEFINE(x,const type __user *, u_obj,...){ 
 if (!check_flow_allowed(&current->s_task,u_obj,obj_type)) do_x(obj,...);}
/// inside KM ///
check_flow_allowed(*s_task,u_obj,obj_type){
s_obj_label* obj= decode(u_obj,obj_type);
if (s_task==NULL && s_obj_label==NULL) return 0;
if(s_obj_label->slist!=NULL)//secrecy flow
 {return check_secrecy_flow(s_task,s_obj_label->slist)}
if(s_obj_label->ilist!=NULL)//integrity flow
 {return check_integrity_flow(s_task,s_obj_label->ilist)}
else // both secrecy and integrity flow
 {return check_safe_flow(s_task,s_obj_label}
}


  
\end{lstlisting}


==> listings/codeml.tex <==
\begin{lstlisting}
static int fn(void* arg) {
  s_execv(mem_obj[1],zlib,deflateInit,Z_DEFAULT_COMPRESSION);
}
void threading_test (void) {
  int cid= s_create(SLABEL);
  int fd= open(tmpname,O_CREAT);
  s_add (cid,persistent_file,fd);
  mem_obj[1] = s_vao_create(DEFAULT, MEMDOM_READ|MEMDOM_WRITE);
  mem_obj[2] = s_vao_create(HW_MD,MEMDOM_READ);
  s_add(cid,vao,memory_obj[1],memory_obj[2])
  // map VA objects to threads
  tid1 = s_clone(cid, mem_obj[1],&fn ,...);
  tid2 = s_clone(cid, mem_obj[2],...);
  s_wait(&status);
  s_cleanup(cid );
}
  
\end{lstlisting}

==> listings/hl.tex <==
\begin{lstlisting}[caption={Pseudocode of using \tool to detect enclave heap leakage},captionpos=b,label={hlcode}]
//-------------Enclave side--------------
void ecall_heap_leak(struct eData* data){
 char temp[] = "kioasdinkadssasdkjhsdaklj";
 char *buf;
 int ret;
 d_enable();//enable tracing
 int mobj=d_create(MMU_MODE,BOUND);
//change malloc -> d_malloc
 data->msg = (char*) d_malloc(mobj,strlen(temp));
 memcpy(data->msg, temp, strlen(temp));
//replaced by Deluminator version of memcpy
 data->len = strlen(temp);
 data->left = strlen(temp);
 while(data->left > 0){
 buf = data->msg + data->len - data->left;
 ocall_write_out(&ret, buf, data->left);
 if(ret <= 0)
    return;
    data->left -= ret;
  }}
//-------------App side--------------
int ocall_write_out(char *buf, int left)
{ printf("%c\n", buf[0]);
  printf("%d\n", left-1);
  return 1;}
int main()
{//init enclave .....//
 d_enable();//enable tracing
 int a_mobj=d_create(MMU_MODE,BOUND);
 struct eData* data = (struct eData*) d_malloc(a_mobj,sizeof(struct eData));
 ret = ecall_heap_leak(eid, data)
  //cleanup enclave......//
}
  
\end{lstlisting}


==> listings/imc.tex <==
\begin{lstlisting}[caption={Internal IMC's data structure },captionpos=b,label={imcstruct}]
struct imc_struct {
    //operation bitmaps: set to 1 if imc[i] 
    //is allowed to do this operation, 0 OW
    DECLARE_BITMAP(imc_Read, IMC_MAX); 
    DECLARE_BITMAP(imc_Write, IMC_MAX);
    DECLARE_BITMAP(imc_Execute, IMC_MAX); 
    DECLARE_BITMAP(imc_Allocate, IMC_MAX);
    int imc_id;    
    struct mutex imc_mutex;
    struct mem_segment *imc_range;
   };
\end{lstlisting}


==> listings/mlexample.tex <==
\begin{lstlisting}
void main (void) {
  compartment c1 = s_create(SLABEL);
  enc_struct e = init_training_enclave(c1);
  s_add (c1, rpc, e->rpc_obj);
  report r = init_attestation(e);
  ....
  init_training(e);
  // rest of the app
  s_cleanup(c1);
}

enc_struct
init_training_enclave(compartment c1) {
  compartment c2 = s_create(SLABEL);
  m_obj m = s_vao_create(DEFAULT, RO);
  shm = s_malloc(m,1024*1024);
  s_add(c2, vao, m_obj);
  init_darknet(c1);
  s_grant(c1->owner, shm);	
}

report
init_attestation(enc_struct e) {
  compartment c3 = s_create(SLABEL);
  m_obj m= s_vao_create(DEFAULT, RO);
  mkeys = s_malloc(m_obj,1024*1024);
  int f_obj = open(fkeys, O_CREAT);
  s_add (c3,persistent_file,f_obj,vao,m);
  t_att = s_clone(c3, m, &do_att...);
}

int do_att(compartment c) {
  // process on attestation keys
  c->mo[1]=keys;
  //process on attestation keys
  write(fkeys, keys, len);
}
\end{lstlisting}

==> listings/mmstruct.tex <==
\begin{lstlisting}[caption={Modifications of mm\_struct },captionpos=b,label={mmstruct}]
struct mm_struct {
...
#ifdef CONFIG_SW_MCA
    struct imc_struct *imc_metadata[IMC_MAX];
    atomic_t num_imc;	/* number of imcs */
    /*imc Page tables per threads.*/
    pgd_t *imc_pgd_list[IMC_MAX];  
    int curr_using_imc;
    spinlock_t sl_imc[IMC_MAX];
    struct mutex imc_metadata_mut;
    DECLARE_BITMAP(imc_InUse, IMC_MAX);
#endif
... };
\end{lstlisting}


==> listings/toctou.tex <==
\begin{lstlisting}[caption={Simple use of \tool for tracing TOCTOU vulnerability on a compartment's file.},captionpos=b,label={toctou}]
d_enable();//enable tracing in this compartment
//add fname to start tracing secrecy violations
//use ILABEL for integrity violations
d_add(fname,file,SLABEL);
//or use open(fname,O_CREAT|SLABEL);
if(!access(fname,W_OK)) {
//Deluminator reports the attacker's TOCTOU e.g., by using symlink to redirect fname
f = fopen(fname,"w+");
operate(f);
...}
else{...}
\end{lstlisting}

==> old/temp.tex <==
\section{Hardening ML Systems}\label{hwe}


 There is a growing need for private computing environments to bridge the gap between strong security/privacy guarantees, and efficient and high-performance edge-cloud computing, in particular for ML and data analytic applications. Private computing (also called confidential computing) contains mechanisms for protecting applications (entirely or partially) from its untrusted host; which can be the host OS, hypervisor, or firmware. By this definition, private computing is a subset of trusted computing that has a broader meaning. Trusted computing explores technology standards as well as the society and government requirements for trusting the next generation of technologies. However, private computing focuses on protecting the confidentiality and integrity of sensitive code and data even in presence of the malicious host. Previous work on software-based \cite{garfinkel2003terra, ta2006splitting, chen2008overshadow, yang2008using, shinagawa2009bitvisor,mccune2008flicker, hofmann2013inktag, zhang2011cloudvisor} and hardware-assisted \cite{baumann2015shielding,tsai2017graphene,guan2017trustshadow,schuster2015vc3,hunt2016ryoan,hunt2018chiron,bittau2017prochlo,bittau2017prochlo} approaches, takes significant steps toward providing private computing environments to a variety of applications. However, as explained in chapter \ref{back}, these systems mostly target private computing on untrusted cloud platforms using legacy hypervisors, and more recently cloud supported hardware enclaves (mainly SGX \cite{anati2013innovative}); that makes them unfit for the fast movement toward pervasive and edge computing on heterogeneous environments with resource constraints. The fundamental issues in performance, efficiency, and compatibility aspects of the existing systems, as well as new attack models \cite{van2018foreshadow, lipp2018meltdown,kocher2018spectre, xu2015controlled,biggio2012poisoning,shokri2017membership,song2017machine}, make this open problem much more challenging than we thought years ago. 
 
 
Despite decades of work, composing systems based on the principle of least privilege is difficult due to the complexity of defining privilege boundaries and the performance challenges they impose. 
To reduce the cost of isolation and TCB (trusted computing base), most hardware platforms already support several isolation layers and memory safety features on the same SoC. For example, Intel supports TXT, SGX, MPX, MPK and more recently TDX that introduces shielded-execution within the hypervisor layer. Hence, between a monolithic design and a least-privilege fully-separated design, there is a vast set of possible compartmentalization boundaries and granularity depending on the security vs. performance trade-offs. However, our traditional OSes, hypervisors, TEE systems, and compartmentalization frameworks are not ready to fully utilize these features simultaneously. Each of the compartmentalization primitives offer limited abstractions. They do not allow developers to explore this continuum of security-performance design points across privilege boundaries. This has lead to a fragmented ecosystem where
developers are building software with over-privileged trust domains and inefficient interaction layers. 

The right abstractions for securely utilizing TEEs/enclaves are still not clear, particularly when combining these hardware features. For instance, depending on the use-cases, various software vendors provide deployment frameworks for running diverse set of workloads within enclaves. Some applications like confidential data analytic benefit from userspace enclaves while other use-cases like micro-services and lightVMs benefit from hypervisor-assisted isolation of trusted domains (TDs). Hence, we see deployment framework, such as Red Hat's Enarx or Amazon Nitro enclaves, which support running the same binary within enclaves in different privilege layers. 
% 
However, the right abstraction at the intersection of these  two layers is unclear in scenarios when \nom{1} enclaves and TDs trust each other; and \nom{2} when they are mutually distrusted. This is challenging particularly since there are open challenges within enclaves itself.
(e.g., over-privilege enclaves, insecure interaction layers). This calls for a bottom-up approach for rethinking our systems stack to enable developers to~\rom{1} effectively utilize these hardware features,~\rom{2} explore the continuum of privilege-performance points across hardware-protection layers, and ~\rom{3} be able to reason about isolation granularity and protect against security threats within interaction layers and other untrusted sources.

First, consider the enclave applications such as 
% To elaborate more, in existing TEE systems, for many use-cases like 
enclave-assisted privacy-preserving data analytic~\cite{grover2018privado,ohrimenko2016oblivious,schuster2015vc3,tramer2018slalom} or web services~\cite{kim2018sgx,hunt2016ryoan}. 
% 
These uses-cases highlight the problem of an over-privileged trust domain, which increases the risk of compromising the enclave~\cite{van2019tale,melara2019enclavedom}. 
% 
An application running in a traditional trusted OS can use 
several software and hardware enabled memory safety features.
% 
However, none of these can be leveraged out-of-the-box inside an enclave. 
% 
Thus, several existing solutions for intra-process isolation are not beneficial for enclaves~\cite{belay2012dune,wangseimi,chen2016shreds,vahldiek2019erim,frassetto2018imix}, despite supporting useful hardware features such as Intel MPK or MPX. The root causes are HW limitations and the tight kernel dependency designed without considering such cross-privilege use cases.

Second, since in-enclave software stack is designed independent than the host OS there is a semantic gap between these independent stacks, so neither layer has sufficient information about the other layers' semantics (e.g., security model, objects and data structure layout, and locations). This semantic gap limits each world's capability to share resources or fully protect itself from the other~\cite{suciu2020horizontal, khandaker2020coin,van2019tale,schwarz2019practical,weichbrodt2016asyncshock,weiser2019sgxjail,SchwarzMichael2017MGEU,machiry2017boomerang}. Thus, it leads to restricted deployment policies which limits the usage and benefits for application developers. In fact, this gap would be worse with the current rise of open-source hardware, which causes even faster progress in hardware-assisted security.
To resolve such issues we need to not only rethink the deployment frameworks (e.g., Enarx or in-enclave LibOSes), but also design OS and hypervisor abstractions for properly introducing these hardware features in a principled way. Only then we can minimize the HW complexity and allow  secure designs to co-exist. 

Next, we discuss our research directions to resolve the above issues in the context of  secure and scalable TDX-assisted systems.


\section{BCI as a usecase}\label{usecase}


\section{Research directions}\label{arch}

We propose a new security architecture with the following building-blocks and abstractions:


\begin{figure*}[h]
    \centering
    \includegraphics[width=1\textwidth,height=3.5in]{images/ideal_ml.pdf}
        \caption{privacy-aware ML system in heterogeneous environments}
\label{fig:idealml}
\end{figure*} 


\begin{itemize}

\item {\todo{lorena}}


\item \textbf{Integrating enclaves \& TDs.}
Users already invest lots of infrastructure (e.g., wasm runtime) and time for ensuring the security of their SGX-assisted applications. However, use-cases like confidential ML encounter relatively large performance overhead due to not being able to use high-performance features inside enclaves or losing some functionalities (fast multi-threading) when compiling to wasm. 
\\
What are the right abstractions for replacing enclaves with TDs or collaborating between them to reduce the performance overhead?
% 
In such deployments, how can we ensure that the security guarantees of sgx-enabled apps are preserved and vice versa? 
% 
Can existing TEE agnostic frameworks (e.g., Google Asylo, Open Enclave SDK, Enarx, Anjuna) support TDX while maintaining the same security guarantees as enclaves?

\item{\textbf{Lightweight units of isolation. }
 Attackers take advantage of inadequate address space isolation within a process or enclave to launch ROP attacks~\cite{lee2017hacking,biondo2018guard,machiry2017boomerang} for extracting secrets or taking control of the enclave. Additionally, insecure shared memory buffers are important attack vectors for extracting secrets or compromising RPC interfaces~\cite{khandaker2020coin}. 
Attackers can launch malicious threads from within the host application process to exploit synchronisation vulnerabilities such as TOCTTOU~\cite{wei2005tocttou,weichbrodt2016asyncshock} or other types of concurrency attacks~\cite{khandaker2020coin} on enclave interfaces. This greatly limits the secure use of enclaves within a multi-threaded application.\\ To resolve these threats, we need new execution units of isolation and abstractions for effective intra-address space isolation which could selectively benefit from minimal hardware support for performance optimization and reducing TCB.
}


\item\textbf{Sufficient privilege separation:} Currently the only solution for sharing systems resources with an enclave is via encrypted channels. Besides the large performance overhead, this approach can not provide additional security (or deprivilege) over already accessed private data or systems object like files. For example, 
a compromised or malicious third-party enclave can collect sensitive data~\cite{schwarz2019practical,marschalek2018wolf} and leak them using OS facilities such as files, network sockets or pipes. 
At the root of such vulnerability classes, there are kernel objects across both the regular and in-enclave worlds which are involved directly (e.g., address space or threads), or indirectly (e.g., files or sockets) to propagate the vulnerability for more damage. 
These objects are an important part of any complex application and 
TEE-assisted applications are no exception. In fact, unlike traditional applications, they rely on these system resources from both worlds. \\ We need a unified security model based on mutual distrust (e.g., difc or object capabilities) for sharing systems resources securely while providing minimal TCB and preserving the original TD's threat model. The result of our previous work shows such full-system compartmentalization is possible with a reasonable overhead~\cite{sirius} which inspired us for reducing the TCB and improving the performance by utilizing TDX.

\item\textbf{Potential Case-studies.}
% Easy deployment} 
% \notezt{remove? over promise}
Solutions like Enarx aim to run unmodified apps on various enclave platforms like AMD's SEV and SGX by providing a lightweight Wasm-based runtime. This approach seems promising for solving portability issues. However, recent works show relatively large performance overhead of wasm apps due to increasing complexity of wasm runtimes for supporting complex applications. The overhead is large particularly when interacting with outside world for I/O operations or multi-threading\cite{jangda2019not}. 
The lack of basic security within wasm linear memory model introduces additional attack vectors~\cite{lehmann2020everything}. We believe integrating our proposed abstractions into a lightweight wasm runtime (e.g., wamr) can significantly mitigate these issues.

% \item\textbf{Side- and covert-channels}\notezt{remove? over promise}

\end{itemize}

==> other.tex <==
% Brain computing technologies have been empowered 
% by the notable progress in computing devices, signal processing, AI, and data analytics. 
% Nowadays, BCI-assisted applications carry a great potential to improve the quality of human lives in medical and non-medical fields. 

%to support people with physical impairments or mental health issues.
% and to develop novel smart environments for education and entertainment.

% particularly beneficial to people who suffer from brain injuries or other disabilities. 
% Moreover, there is an increasing number of 
% wearable BCI use cases for better monitoring health, mental/emotional state (e.g., focus, anxiety, or motivation), or sleep quality~\cite{lakhan2019consumer,abdulkader2015brain}.

% The aforementioned examples are only a small subset of what could ultimately be available in the near future.


% Adequate security and privacy protections in such applications are extremely crucial. 

%Major attack vectors, ranging from access control and privilege management to adversarial machine learning (ML), are overlooked by existing BCI frameworks. 
% Our investigation on real-world BCI devices and applications shows a disappointing state in their security and privacy practices. 

% For instance, inadequate access control management allows a malicious process to access/alter raw EEG data, sensitive ML predictions, or associated peripherals (e.g., GPIOs of BCI-controlled devices).

% These risks become even higher with the wide use of transfer learning due to the ability to transfer malicious intentions together with the learnt features of the pre-trained model~\cite{gu2019badnets}.

%Our investigation on real-world BCI frameworks and applications (\S\ref{sec:eval}) shows such severe attack vectors are entirely overlooked. The first step for developing protection is detecting and analyzing such security and privacy threats. This is challenging without proper tooling, particularly for non-expert developers. Additionally, combining various methods for supporting each attack vector leads to a complex and costly solution that is not suitable for resource-constrained BCI-edge devices.

%Hence, we propose \tool, an extensible \textit{domain-specific} framework for helping developers to investigate various attack vectors when building BCI applications. To provide a lightweight solution, \tool is optimized based on the security, privacy, and resource requirements of contemporary BCI-mobile applications.
% 
%why BCI-specifi solution? (1) bci is safty-critical, (2) well-defined complex-attack surface that despite being dficult its still feasible, efficient due to resource constraint
%\notezt{this is an modular extensible framwwork, we only use the 6 attack category as PoCs but other attacks are possible to be investigated too}
%\notezt{developers struggle to design secure sytsems due to lack of proper tooling and developer-frindly env~\cite{chowdhury2021developers}} 
%\lorena{advertise here the mapping of ML and system}
% 
% 

%One of our main observations is that domain-specific IFC systems can resolve these issues and provide efficient, strong, and fine-grained security guarantees suitable for resource-constrained devices.

%Likewise, various systems proposed security platforms or analyses of smart homes~\cite{lei2020secwir,fernandes2016security} or automobiles~\cite{checkoway2011comprehensive}.

% The infinite potentials of BCIs can, therefore, be hindered by significant security and privacy threats, which are highly overlooked by the current BCI-edge platforms.
%Current general-purpose approaches are not easily adoptable since they offer complex solutions that aim (and fail) to cover the vast pool of mobile/IoT security threats. They also introduce unnecessary computational and programmability overheads.
% 
% Moreover, since the current state of mobile/IoT security threats is too vast for a general-purpose solution, we present a BCI-edge specific approach.
% 
% Existing solutions are not easily adoptableThe current state of mobile/IoT security threats is too vast for a general-purpose solution
%

% BCI applications are often enhanced by connecting to mobile phones or IoT devices, and rely on machine learning techniques for interpreting brain signals.

%BCI applications often involve connecting to mobile phones or IoT devices, relying on insecure software dependencies, and ML-based data processing. Consequently, they are susceptible to a complex set of attacks that are highly overlooked by the current BCI-edge platforms.

==> results/datasets.tex <==
\section{Datasets}

==> results/malloc.tex <==
 \begin{figure}[t]

 \begin{tikzpicture}
    \begin{axis}[
         width=0.5\textwidth,
        height=4cm,
        bar width=4.2pt,
        % commented to see, if the result is correct
%        major x tick style=transparent,
        symbolic x coords={1,2,4,8,16,32,64,128,256,512},
        %enlarge x limits=0.5,
        xlabel={Allocated Memory (KB)},
        xtick=data,
        %x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
        % changed from `\pgflinewidth' to 1 easier see that the result is correct
        ymin=0,
         ymax=15,
        % changed to 0 to make the computation of the shift easier
        ybar=0pt,
        ymajorgrids=true,
        ylabel={Latency(ms)},
        legend cell align=left,
        legend style={
            at={(1,1.05)},
            legend columns=3,
            anchor=south east,
            column sep=1ex
        },
    ]
        % add a scope around the to shift bars
        \begin{scope}[
            % shift the bars accordingly
            xshift={0.1*\pgfplotbarwidth},
            % and just "fill" the bars
            % (to avoid overlapping of the more right bars to the more left ones)
            draw=none,
        ]
            % your style could heavily be simplified to just providing the `+'
            % sign and the color as option
            %\addplot+ [bblue]  coordinates
             %   {(St.~2,10006) (St.~3,99895) (St.~4, 99867)};
            %\addplot+ [rred]   coordinates
             %   {(St.~1,1) (St.~2,10006) (St.~3,99448) (St.~4, 99487)};



\addplot+ [draw=none, fill=torange,
            error bars/.cd,
                y dir=both,
                % (changed from `y explicit` so the error bars are (clearly) visible
                y explicit relative,
        ] coordinates {
            (1,10.12) +- (0,0.09)
            (2,9.80) +- (0,0.1)
            (4,10.12) +- (0,0.09)
            (8,10.08) +- (0,0.1)
            (16,9.66) +- (0,0.1)
            (32,9.42) +- (0,0.1)
            (64,10.61) +- (0,0.08)
            (128,10.18)  +- (0,0.09)
            (256,10.47) +- (0,0.09)
            (512,10.43) +- (0,0.09)
        };
        
        \addplot+ [draw=none, b1,
            error bars/.cd,
                y dir=both,
                % (changed from `y explicit` so the error bars are (clearly) visible
                y explicit relative,
        ] coordinates {          
            (1,9.13) +- (0,0.13)
            (2,9.12) +- (0,0.13)
            (4,8.7) +- (0,0.13)
            (8,9.04) +- (0,0.13)
            (16,9.15) +- (0,0.12)
            (32,9.03) +- (0,0.13)
            (64,10.44) +- (0,0.09)
            (128,10.27)  +- (0,0.1)
            (256,11.30) +- (0,0.08)
            (512,12.12) +- (0,0.09)
                        };
        


        \end{scope}

\legend{Native, \tool-app}
    \end{axis}
\end{tikzpicture}
\caption{Cost of tracking memory regions using \tool's memory management API (\texttt{a\_malloc/a\_free}).}

\label{tab:smalloc}
 \end{figure}
 


==> tables/att.tex <==
\begin{table*}
\resizebox{2\columnwidth}{!}{%

    \begin{tabular}{|l|l|l|l|}
    \hline
    Attack       & Description          & Labeled objs (enclave)              & Labeled objs (host)        \\ \hline
    tale~\cite{van2019tale}                       & mem cor in ABI       & VA obj, RPC         & -                                          \\ \hline
    Async~\cite{weichbrodt2016asyncshock}                     & concurrency          & thrd, VA obj, RPC  & thrd,RPC                  \\ \hline
    Boomerang~\cite{machiry2017boomerang}                  & Exec Overflow   & thrd, VA obj, RPC  & thrd, VA obj, RPC           \\ \hline
    HPE~\cite{suciu2020horizontal}                       & Priv escalation      & thrd, RPC               & thrd, file,RPC                  \\ \hline
    Diamorphine~\footnote{https://github.com/m0nad/Diamorphine} & malware/Iago & detected by \ssm                                 & detected by \ssm                                       \\\hline
        mirai~\footnote{https://github.com/0x27/linux.mirai}& malware/Iago & detected by \ssm                                   & detected by \ssm                                       \\\hline
        
       Nailgun~\footnote{https://compass.cs.wayne.edu/nailgun} & malware/Iago & detected by \ssm                                  & detected by \ssm                                          \\\hline
    \end{tabular}}
\end{table*}

% attack
% attack name/cve
% attacker
% victim
% description/attack vector(s): corrupt kernel stack, inject code in the kernel, return bad syscall value
% impact: confidentiality, integrity, leak keys, change enclave control flow
% defense
% labeled objects 
% detected violation: fails integrity check by ssm at boot, at runtime, flow from x to y, 


% requirement:
% no code injection
% cannot break cfi or dfi
% bug in the kernel
% corrupts data
% this data will be sent to the enclave 

% example flow for iago:
% enclave - create file f
% kernel - done
% enclave - open, write, close
% kernel - ok
% enclave - open file
% kernel checks, creates id
% attacker corrupts data and overwrites return code with error
% kernel file - doesnt exist
% enclave - ok, create new file

==> tables/att2.tex <==
\begin{table*}[t]
\resizebox{2.1\columnwidth}{!}{%
   \begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
    \textbf{Source/Project} & \textbf{Attacker} & \textbf{Victim}  & \textbf{Description}  & \textbf{Compartments Objects} & \textbf{Policy Violation}  & \textbf{LoC} & \textbf{Over}\\ \hline
    
   
      
        COIN~\cite{khandaker2020coin} &   host app   &   enclave    & heap info leak  &  $C1\{t_e,mo, ocall\}$ $C2\{t_a,ocall\}$&  $ t_e \not\longrightarrow ocall(mo)\not\longrightarrow t_a$  & 5   &   14\%                         \\ \hline
        
         COIN~\cite{khandaker2020coin} &   host app   &   enclave    &   malicious calls  &  $C1\{t_e,mo_e, rpc\}$ $C2\{t_a,mo_a, rpc\}$&  $ t_a^{\otimes} \not\longrightarrow ecall(mo_a) \quad t_e \not\longrightarrow ocall(mo_e)$  & 9   &   17\%                         \\ \hline

       COIN~\cite{khandaker2020coin} &   host app   &   enclave    & heap overflow  &  $C1\{t_e,mo, rpc\}$ $C2\{t_a,rpc\}$&  $ t_e \not\longrightarrow ocall(mo)\not\longrightarrow t_a$  & 6   &   14\%                         \\ \hline
       
       
       SGX-tls~\cite{zhang2019sgx} &   host app   &   enclave    & stack info leak &  $C1\{t_e^1,mo^1\}$ $C2\{t_e^2,mo^2\}$& $t_e^1\not\longrightarrow mo^2 (memcpy(mo^2,mo^1,size))$  & 21   &   18\%      \\ \hline 
  

    SGX_SQLite~\cite{mazhkenovsgx}& host app   &  enclave   &  malicious calls & $C1\{t_e^1,f_e\}$ $C2\{t_a\}$  & $t_a^{\otimes} \not\longrightarrow f_e^$    &  8  &  13\%         \\ \hline
    
  
    
    SGX-Tor~\cite{kim2018sgx}& enclave   &  host app   & export secret  & $C1\{t_e,mo\}$ $C2\{t_u,f_u,s_u,p_u\}$& $t_e{\otimes} \not\longrightarrow \{t_u,f_u,s_u,p_u\}$   &  15  &    21\%       \\ \hline
     SGX-Tor~\cite{kim2018sgx}& host app   &  enclave & concurrent calls  & $C1\{t_e\}$ $C2\{t_a\}$& $t_a^{\otimes} \not\longrightarrow \{t_e\}$   &  4  &    9\%       \\ \hline
          Boomerang~\cite{machiry2017boomerang}     & host app        & TA/kernel    & break TZ-OS         & $C1\{t_e,mo_e, rpc_e\}$ $C2\{t_a,mo_e,rpc_e\}$            &  $t_a^{\otimes} \not\longrightarrow mo_e$   & 23  &    13\%           \\ \hline
    OPTEE~\cite{optee}& host app   &  TA   &  TA mem corr    & $C1\{t_e^1,mo_e\}$ $C2\{t_e^2\}$ &   $t_e^2 \not\longrightarrow mo_e$ &  8 &    13\%        \\ \hline
    OPTEE~\cite{optee}& TA   &  TA   &  memory leak    & $C1\{t_e\}$ $C2\{t_a,mo\}$ &   $t_e \not\longrightarrow mo$ &  11 &    13\%        \\ \hline
   OPTEE~\cite{optee}& host app   &  TA   & TA mem leak    & $C1\{t_e,mo_e,rpc_e\}$ $C2\{t_a\}$ &   $t_a \not\longrightarrow rpc_e(mo_e)$ &  9 &    12\%        \\ \hline

     
    tale~\cite{van2019tale}       & host app       & enclave      & enclave mem corr       & $C1\{t_e,mo_e^1, rpc_e\}$ $C2\{t_a,rpc_e\}$ &  $t_e^{\otimes} \not\longrightarrow mo_e^1 \quad t_a^{\otimes} \not\longrightarrow t_e$  & 12   &                            \\ \hline
    
    async~\cite{weichbrodt2016asyncshock}      & host app        & enclave       & concurrency          & $C1\{t_e,mo_e, rpc_e\}$ $C2\{t_a,mo_a,rpc_e\}$              & $t_a^{\otimes} \not\longrightarrow rpc_e \quad t_a^{\otimes} \not\longrightarrow mo_e \land mo_a$  & 18       &         \\ \hline
    
    HPE~\cite{suciu2020horizontal}     & host app        & other app       & break shared enclave        & $C1\{t_e, rpc_e^1,rpc_e^2\}$ $C2\{t_a,rpc_e\}$              & $t_a^{\otimes} \not\longrightarrow rpc_e^2$      & 9  &           \\ \hline
    

   
    \end{tabular}

}
\caption{Utilizing \tool for investigating vulnerabilities across privilege boundaries. We use subscripts $e$ for enclave objects, $a$ for app, $u$ for untrusted host source, $\otimes$ for attacker,  $t$ for thread, $mo$ for memory object, $rpc$ for RPC object that means ocalls/ecalls, $f$ for file/db,$s$ for socket, $p$ for pipe,$\not\longrightarrow$ for dataflow policy violation. }
\label{tab:detect}
\end{table*}

==> tables/difc-rules.tex <==
\begin{table}[H]
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{|l|l|}
    \hline
     Secrecy dataflow $p$ to $q$ & $\{S_{p}-D_{p} \subseteq{S_{q} \cup D_{q}} \}$ \\ \hline
     Integrity dataflow $p$ to $q$ & $ \{I_{q}-D_{q} \subseteq{I_{p} \cup D_{p}} \}$ \\ \hline
      Safe data flow $p$ to $q$ &  $\{S_{p}-D_{p} \subseteq{S_{q} \cup D_{q}} \} \land \{I_{q}-D_{q} \subseteq{I_{p} \cup D_{p}} \}$ \\ \hline
      Safe label change $L$ to $L'$ &  $\{L'-L\}^{+} \cup \{L-L'\}^- \subseteq{C_{p}}$ \\ \hline

    \end{tabular}}
    \caption{Summary of \tool dataflow policies.}
    \label{tab:difc}
    \squeezeup

\end{table}




==> tables/domains.tex <==

\begin{table}[]
\resizebox{\columnwidth}{!}{%

    \begin{tabular}{|l|l|l|}
    
    \hline
    Mode & Bits & Description                                                                     \\ \hline
    No Access   & 00 &  Any access causes a domain fault.                          \\\hline
    Manager     & 11 & Full accesses with no permissions check.\\\hline
    Client      & 01 &  Accesses are checked against page tables   \\\hline
    Reserved    & 10 &   Unknown behaviour. \\ \hline
    \end{tabular}}
    \caption{ARM memory domains access permissions }
    \label{domains}
\end{table}


==> tables/extra.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{.8}
    \begin{tabular}{|ll|}
    \hline
    \textbf{Common enclave operations: }                                               & ~                                                    \\
    \texttt{s\_create\_enclave $\rightarrow$ eid}                                                  & create an enclave                                    \\
    \texttt{s\_ecall (rpc\_msg *, arguments)}                        & call from the host thread to the enclave             \\
      \texttt{s\_ocall (rpc\_msg *, arguments)}                      & call from the enclave to the host thread             \\
      \texttt{s\_delete\_enclave(eid)}                                      & delete an enclave                                    \\ \hline
      \textbf{Common security policy syscalls : }& ~                                                    \\
      \texttt{s\_grant/revoke (label\_info *, tid, dir)}                        & give/revoke thread privileges to objects           \\
      \texttt{s\_access\_enable/disable (label\_info *)}                                     & enable/disables access to set of objects                    \\
      \texttt{s\_clone (label\_info *,...) $\rightarrow$ tid}                                           & create a labeled child                               \\
      \texttt{open/socket/pipe(label\_info *,...) $\rightarrow$ ret}                                    & create a labeled kernel object                       \\ \hline
   \textbf{ API for Address space isolation:  }                                  & ~                                                    \\
      \texttt{imc\_create(hw-mode-flags) $\rightarrow$ imc\_id}                                            & create a new IMC (kernel- or hardware-backed)        \\
      \texttt{imc\_grant/revoke(imc\_id, P)}                                            & grants/revoke IMC the capability to imc with priv P        \\
      \texttt{imc\_malloc/free(imc\_id, ...)}                                         & allocate/deallocate memory within an imc                       \\
      \texttt{imc\_mprotect/mmap/munmap(imc\_id,...)}                                       & add/remove pages or change its  permission \\
      \texttt{imc\_kill(imc\_id)}                                                             & cleanup an IMC                                       \\ \hline
    \end{tabular}
    \caption{Summary of the Sirius application interface}
    \label{scapi}
\end{table*}


==> tables/ml.tex <==

\begin{table}[tp]
\centering

\resizebox{.6\columnwidth}{!}{%
    \begin{tabular}{|l|c|c|}
    \hline
    Operation       &       {Native} & {\tool}    \\ \hline
     training        & 75.234 s & 78.486 s     \\ \hline
    pre-trained           &  6.8753 s & 7.3987 s   \\ \hline
    inference         &  33.23 \textmu s & 36.32 \textmu s \\ \hline

    \end{tabular}
    
    }
 
  \caption{Latency overhead of Darknet ML framework.}
     \label{tab:darknet}
\end{table} 


==> tables/optee.tex <==
\begin{table}[tp]
\sisetup{separate-uncertainty}
\centering
 \resizebox{0.8\columnwidth}{!}{%
\begin{tabular}
  {@{} 
    l
    S[table-format = 3.2(2)]
    S[table-format = 3.2(2)]
    S[table-format = 3.2(2)]
  @{}}
  \toprule
    & \multicolumn{2}{c}{Latency ({\textmu s})} \\
    &  \multicolumn{1}{c}{OP-TEE} & {Sirius SK}  \\
  \midrule
      create enclave          & 99.82(2)            &     93.95(1)   \\
    delete enclave         &    30.02(1)   &      30.10(1)  \\
     enclave calls (ecall ocall)         &  22.68 (1)     &    20.14(3) \\
     shared memory & 9.58(2) ms & 8.16(1) ms \\
     file system (read/write) & 375.8(3) ms& 34.68(1) ms\\
%     allocating shared memory & 10.41(3) & 8.75(2) \\
  \bottomrule
\end{tabular}}
\caption{Average overhead ($20000$ runs) comparison of enclave operations in \tool vs OP-TEE.}
\label{tab:optee}
\end{table}


==> tables/tb1.tex <==
\begin{table}[t]

\footnotesize
\newcommand*\rot[1]{\hbox to1em{\hss\rotatebox[origin=br]{-30}{#1}}}
\newcommand*\feature[1]{\ifcase#1 -\or\LEFTcircle\or\CIRCLE\fi}
\newcommand*\f[4]{\feature#1&\feature#2&\feature#3&\feature#4&\fcontinued}
\newcommand*\fcontinued[1]{\feature#1}
\makeatletter
\newcommand*\ex[4]{#1\tnote{#2}&#3&%
    \f#4&\@firstofone
}
\makeatother
\newcolumntype{G}{ccc}
\begin{threeparttable}
\centering
 \resizebox{0.8\columnwidth}{!}{%

\begin{tabular}{@{}lc GG !{\kern.1em} GG !{\kern.1em} GG@{}}
\toprule
Security mechanisms &   & \multicolumn{3}{c}{Security Principles} \\
\midrule
% rotated items
 && \rot{P0}
 & \rot{P1}
  & \rot{P2}
  & \rot{P3}
 & \rot{P4}
 \\
\midrule
\ex{ACM~\cite{setools,seccomp,sandhu1994access,watson2003trustedbsd}}{}{}  {11000}\\
\ex{Object capability\cite{shapiro1999eros,watson2015cheri,watson2012taste}}{}{}  {22111}\\
\ex{IFC\cite{denning1976lattice,mcilroy1992multilevel,fraser2000lomac,yumerefendi2007tightlip}}{}{}  {11111}\\
\ex{DIFC-OSes~\cite{myers2000protecting,zeldovich2006making,krohn2007information}}{}{}  {21121}\\
\ex{\codename}{}{}  {22222}\\



\bottomrule
\end{tabular}}
\begin{tablenotes}
\item $\feature2$ { }{ }{ } practical, $\feature1$ { }{ }{ } large overhead 
 $\text{{ }\feature0}$ { }{ }{ } partial/not feasible
\end{tablenotes}   
\end{threeparttable}
\caption{{Feasibility and practicality of using existing security models to achieve \codename security principles.}}
\label{tab:properties}

\end{table}



==> tables/thrd.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%

    \begin{tabular}{|l|c|c|c|c|}
    \hline
    Operation       &       {fork} & {pthread} & {s\_clone} & {hw s\_clone}    \\ \hline
    Launch (1MB)        & 280.24 & 31.17 & 51.80 & 31.98  \\ \hline
    Join (1MB)            &  832.45 &  1.10  & 3.78 &  1.70  \\ \hline
    Launch (2MB)         &  331.40 & 31.51 & 51.85 & 32.1 \\ \hline
    Join (2MB)         &  1126.69& 1.13 & 3.82(3) & 1.78 \\ \hline

    \end{tabular}}
    \caption{Average latency overhead of \tool threading. }
        \label{tab:thrdproblem}
\end{table}

